Distributed Spectrum Access with Spatial Reuse

Efficient distributed spectrum sharing mechanism is crucial for improving the spectrum utilization. The spatial aspect of spectrum sharing, however, is less understood than many other aspects. In this paper, we generalize a recently proposed spatial congestion game framework to design efficient distributed spectrum access mechanisms with spatial reuse. We first propose a spatial channel selection game to model the distributed channel selection problem with fixed user locations. We show that the game is a potential game, and develop a distributed learning mechanism that converges to a Nash equilibrium only based on users' local observations. We then formulate the joint channel and location selection problem as a spatial channel selection and mobility game, and show that it is also a potential game. We next propose a distributed strategic mobility algorithm, jointly with the distributed learning mechanism, that can converge to a Nash equilibrium.

==> Algorithm.tex <==
\newpage

\begin{table*}
\hrule
\vspace{0.3cm}
\caption{\label{alg:Distributed-Learning-For}Distributed Learning For Spatial Channel Selection}
%\vspace{-0.3cm}
\hrule
\begin{algorithmic}[1]
\State \textbf{initialization:}
\State \hspace{0.4cm} \textbf{set} the initial perception value $\boldsymbol{Z}_{n}(0)=(\frac{1}{M},...,\frac{1}{M})$, and the period index $T=0$.
\State \textbf{end initialization\newline}

\Loop{ for each decision period $T$ and each user $n$ in parallel:}
        \State \textbf{select} a channel $a_{n}(T)\in\mathcal{M}$ according to (\ref{eq:DL-0}).
        \For{each time slot $t$ in the period $T$}
            \State \textbf{sense} and \textbf{contend} to access the channel $a_{n}(T)$.
            \State \textbf{record} the realized utility $\tilde{U}_{n}(T,t)$
        \EndFor
        \State \textbf{calculate} the average utility $\tilde{U}_{n}(T)=\frac{\sum_{t=1}^{K}\tilde{U}_{n}(T,t)}{K}$.
        \State \textbf{update}  the perception values $\boldsymbol{Z}_{n}(T)$ according to (\ref{eq:DL-1}).
        \State \textbf{set} the period index $T=T+1$.
\EndLoop
\end{algorithmic}
\hrule
\end{table*}


\begin{table*}
\hrule
\vspace{0.3cm}
\caption{\label{alg:Distributed-Strategic-Mobility}Distributed Strategic Mobility Algorithm}
%\vspace{-0.3cm}
\hrule
\begin{algorithmic}[1]
\State \textbf{initialization:}
\State \hspace{0.4cm} \textbf{set} the temperature $\gamma$ and the timer density $\tau$.
\State \textbf{end initialization\newline}

\Loop{ for each user $n$ in parallel:}
        \State \textbf{generate}  a timer value that follows the exponential distribution
with the mean equal to $\frac{e^{\tau}}{|\mathcal{\triangle}_{d_{n}}^{n}|}$,
where $d_{n}$ is the current location of the user and $|\mathcal{\triangle}_{d_{n}}^{n}|$
is the number of feasible locations to move to next.
        \State \textbf{count down} until the timer expires.
        \If{ the timer expires}
            \State \textbf{record} the payoff $U_{n}(D,A)$.
            \State \textbf{choose}  a new location $d_{n}^{'}$ randomly from the set $\mathcal{\triangle}_{d_{n}}^{n}$.
            \State \textbf{move} to the new location $d_{n}^{'}$ and \textbf{record} the payoff $U_{n}(D^{'},A)$.
            \State \textbf{stay in}  the new location $d_{n}^{'}$
with probability $\frac{e^{-\log(1-p_{n})\gamma U_{n}(D^{'},A)}}{e^{-\log(1-p_{n})\gamma U_{n}(D,A)}+e^{-\log(1-p_{n})\gamma U_{n}(D^{'},A)}}$
OR \textbf{move back} to the original location $d_{n}$ with probability $\frac{e^{-\log(1-p_{n})\gamma U_{n}(D,A)}}{e^{-\log(1-p_{n})\gamma U_{n}(D,A)}+e^{-\log(1-p_{n})\gamma U_{n}(D^{'},A)}}$.
        \EndIf
\EndLoop
\end{algorithmic}
\hrule
\end{table*}

%\begin{algorithm}[tt]
%\begin{algorithmic}[1]
%\State \textbf{initialization:}
%\State \hspace{0.4cm} \textbf{set} the temperature $\gamma$ and the timer density $\tau$.
%\State \textbf{end initialization\newline}
%
%\Loop{ for each user $n$ in parallel:}
%        \State \textbf{generate}  a timer value that follows the exponential distribution
%with the mean equal to $\frac{e^{\tau}}{|\mathcal{\triangle}_{d_{n}}^{n}|}$,
%where $d_{n}$ is the current location of the user and $|\mathcal{\triangle}_{d_{n}}^{n}|$
%is the number of feasible locations to move to next.
%        \State \textbf{count down} until the timer expires.
%        \If{ the timer expires}
%            \State \textbf{record} the payoff $U_{n}(D,A)$.
%            \State \textbf{choose}  a new location $d_{n}^{'}$ randomly from the set $\mathcal{\triangle}_{d_{n}}^{n}$.
%            \State \textbf{move} to the new location $d_{n}^{'}$ and \textbf{record} the payoff $U_{n}(D^{'},A)$.
%            \State \textbf{stay in}  the new location $d_{n}^{'}$
%with probability $\frac{e^{-\log(1-p_{n})\gamma U_{n}(D^{'},A)}}{e^{-\log(1-p_{n})\gamma U_{n}(D,A)}+e^{-\log(1-p_{n})\gamma U_{n}(D^{'},A)}}$
%OR \textbf{move back} to the original location $d_{n}$ with probability $\frac{e^{-\log(1-p_{n})\gamma U_{n}(D,A)}}{e^{-\log(1-p_{n})\gamma U_{n}(D,A)}+e^{-\log(1-p_{n})\gamma U_{n}(D^{'},A)}}$.
%        \EndIf
%\EndLoop
%\end{algorithmic}
%\caption{\label{alg:Distributed-Strategic-Mobility}Distributed Strategic Mobility Algorithm}
%\end{algorithm}


%\begin{algorithm}[tt]
%\begin{algorithmic}[1]
%\State \textbf{initialization:}
%\State \hspace{0.4cm} \textbf{set} the initial perception value $\boldsymbol{Z}_{n}(0)=(\frac{1}{M},...,\frac{1}{M})$, and the period index $T=0$.
%\State \textbf{end initialization\newline}
%
%\Loop{ for each decision period $T$ and each user $n$ in parallel:}
%        \State \textbf{select} a channel $a_{n}(T)\in\mathcal{M}$ according to (\ref{eq:DL-0}).
%        \For{each time slot $t$ in the period $T$}
%            \State \textbf{sense} and \textbf{contend} to access the channel $a_{n}(T)$.
%            \State \textbf{record} the realized utility $\tilde{U}_{n}(T,t)$
%        \EndFor
%        \State \textbf{calculate} the average utility $\tilde{U}_{n}(T)=\frac{\sum_{t=1}^{K}\tilde{U}_{n}(T,t)}{K}$.
%        \State \textbf{update}  the perception values $\boldsymbol{Z}_{n}(T)$ according to (\ref{eq:DL-1}).
%        \State \textbf{set} the period index $T=T+1$.
%\EndLoop
%\end{algorithmic}
%\caption{\label{alg:Distributed-Learning-For}Distributed Learning For Spatial Channel Selection}
%\end{algorithm}

==> POA.tex <==

\section{Uniqueness and Efficiency of Nash Equilibrium}\label{POA}

In previous sections, we have considered the existence of Nash equilibrium and proposed distributed algorithms for achieving the equilibrium. We will further explore the uniqueness and efficiency of the Nash equilibrium, which can offer more useful insights for the game theoretic approach for distributed spectrum sharing with spatial reuse.

\subsection{Uniqueness of Nash equilibrium}

Due to the combinatorial nature of joint channel and location
selections, the Nash equilibrium of the game  is not unique in general.
For example, we consider a game with two users $\mathcal{N}=\{1,2\}$, two channels
$\mathcal{M}=\{1,2\}$, and two locations $\Delta=\{d^{1},d^{2}\}$.
Two locations are close such that $||d^{1},d^{2}||\leq\delta$, and
both users and channels are homogeneous such that $\theta_{m}=\theta,B_{m,d_{n}}^{n}=B,p_{n}=p$.
In this case, there are eight Nash equilibria $((d_{1},d_{2}),(a_{1},a_{2}))$ for the game, i.e.,
$\left(\left(d^{1},d^{1}\right),\left(1,2\right)\right)$, $\left(\left(d^{2},d^{2}\right),\left(1,2\right)\right)$,
$\left(\left(d^{1},d^{1}\right),\left(2,1\right)\right)$, $\left(\left(d^{2},d^{2}\right),\left(2,1\right)\right)$,$\left(\left(d^{1},d^{2}\right),\left(1,2\right)\right)$,
$\left(\left(d^{1},d^{2}\right),\left(2,1\right)\right)$,
$\left(\left(d^{2},d^{1}\right),\left(1,2\right)\right)$, and $\left(\left(d^{2},d^{1}\right),\left(2,1\right)\right)$.

In general, selecting from multiple Nash equilibria is quite hard, and the proposed algorithm is guaranteed to converge to one of the Nash equilibria.


\subsection{Price of Anarchy}

Since the Nash equilibrium is typically not unique, we then study the efficiency of Nash equilibria. Following the
definition of price of anarchy (PoA) in game theory \cite{key-16}, we will quantify
the efficiency ratio of the worst-case Nash equilibrium over the centralized optimal solution. We first consider the spatial channel selection game with
a fixed spectrum access location profile $\boldsymbol{d}$. Let $\Xi$
be the set of Nash equilibria of the game. Then the PoA is defined
as\[
\mbox{PoA}=\frac{\min_{\boldsymbol{a}\in\Xi}\sum_{n\in\mathcal{N}}U_{n}(\boldsymbol{d},\boldsymbol{a})}{\max_{\boldsymbol{a}\in\mathcal{M}^{N}}\sum_{n\in\mathcal{N}}U_{n}(\boldsymbol{d},\boldsymbol{a})},\]
which is always not greater than $1$. A larger PoA implies that the set of Nash equilibrium is more efficient (in the worst-case sense) using the centralized optimum as a benchmark. Let $\varpi=\max_{n\in\mathcal{N}}\{-\log(1-p_{n})\}$,
$E(\boldsymbol{d})=\min_{n\in\mathcal{N}}\max_{m\in\mathcal{M}}\left\{ \log\left(\theta_{m}B_{m,d_{n}}^{n}p_{n}\right)\right\} $,
and $K(\boldsymbol{d})=\max_{n\in\mathcal{N}}\{|\mathcal{N}_{n}(\boldsymbol{d})|\}$. We can show that
\begin{thm}
\label{thm:For-the-spatialPoA}For the spatial channel selection game
with a fixed spectrum access location profile $\boldsymbol{d}$, the
PoA is no less than $1-\frac{K(\boldsymbol{d})\varpi}{E(\boldsymbol{d})}$.\end{thm}

The proof is given in Appendix \ref{proofPoA}. Intuitively, when users are less aggressive in channel contention (i.e., $\varpi$ is smaller) and users are more homogeneous in term of channel utilization (i.e., $E(\boldsymbol{d})$ is larger), the worst-case Nash equilibrium is closer to the centralized optimum and hence the PoA is larger.  Moreover, Theorem \ref{thm:For-the-spatialPoA} implies that we can increase the efficiency of spectrum sharing  by better utilizing the gain of spatial reuse (i.e., reducing the interference edges
$K(\boldsymbol{d})$ on the interference graph). Similarly, by defining
that $\eta=\max_{\boldsymbol{d}\in\Theta}\{\frac{K(\boldsymbol{d})}{E(\boldsymbol{d})}\}$,
we see that the PoA of the joint spatial channel selection and mobility game is no less than $1-\eta\varpi$.

The PoA characterizes the worst-case performance of Nash equilibria. Numerical results in Section \ref{sec:Numerical-Results} demonstrate that the convergent Nash equilibrium of the proposed algorithm is often more efficient and has a less than $8\%$ performance loss,
compared with the centralized optimal solution.

